Plucker Formulas for Plane Algebraic Curves with a Given Newton Polygon

Let $C$ be a generic complex plane plane curve with a given Newton polygon $P$. We compute the number of its inflection points and bitangents (equivalently, the number of singularities of the projectively dual curve $C^\vee$). We also prove that $C^\vee$ has no singularities other than nodes and cusps for large enough polygons $P$.

==> pic/bitangdiagrams.tex <==
\begin{tikzpicture}[scale=0.5]
	\initver
	\draw[step=1,black!20,very thin] (-0.4,-0.4) grid (4.4,4.4);
	\draw[black,dashed, thick] (0, 0) -- (0,4) -- (4,0) -- cycle;
	\node at (0,0) [ver] {};
	\node at (1,0) [ver] {};
	\node at (2,0) [ver] {};
	\node at (3,0) [ver] {};
	\node at (4,0) [ver] {};
\end{tikzpicture}

==> pic/infldiagrams.tex <==
\begin{tikzpicture}[scale=0.5]
	\initver
	\draw[step=1,black!20,very thin] (-0.4,-0.4) grid (3.4,3.4);
	\draw[black,dashed, thick] (0, 0) -- (0,3) -- (3,0) -- cycle;
	\node at (0,0) [ver] {};
	\node at (1,0) [ver] {};
	\node at (2,0) [ver] {};
	\node at (3,0) [ver] {};
\end{tikzpicture}

